MentalImager: Exploring Generative Images for Assisting Support-Seekers' Self-Disclosure in Online Mental Health Communities

Support-seekers' self-disclosure of their suffering experiences, thoughts, and feelings in the post can help them get needed peer support in online mental health communities (OMHCs). However, such mental health self-disclosure could be challenging. Images can facilitate the manifestation of relevant experiences and feelings in the text; yet, relevant images are not always available. In this paper, we present a technical prototype named MentalImager and validate in a human evaluation study that it can generate topical- and emotional-relevant images based on the seekers' drafted posts or specified keywords. Two user studies demonstrate that MentalImager not only improves seekers' satisfaction with their self-disclosure in their posts but also invokes support-providers' empathy for the seekers and willingness to offer help. Such improvements are credited to the generated images, which help seekers express their emotions and inspire them to add more details about their experiences and feelings. We report concerns on MentalImager and discuss insights for supporting self-disclosure in OMHCs.

==> Draft/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/0_abstract.tex <==


\begin{abstract}
\pzh{
Support-seekers' self-disclosure of their suffering experiences, thoughts, and feelings in the post can help them get needed peer support in online mental health communities (OMHCs). 
However, such mental health self-disclosure could be challenging.
Images can facilitate the manifestation of relevant experiences and feelings in the text; yet, relevant images are not always available.
% In this paper, we explore generative images for assisting support-seekers' self-disclosure in OMHCs. 
% We first examine the feasibility of [...] for generating 
In this paper, we present a technical prototype named MentalImager that can generate topical- and emotional-relevant images based on the seekers' drafted posts or specified keywords. 
Results from a within-subjects study (N=24) indicate that MentalImager can improve seekers' satisfaction with the self-disclosure in their posts and increase support-providers' willingness to offer help. 
The generated images help seekers express their emotions and stimulate them to add more details about their experience, which improves providers' empathy and understanding of the seekers.
We report concerns on MentalImager and discuss insights for supporting self-disclosure in OMHCs.
}
    % The text-based Online Mental Health Communities (OMHCs) provide an effective means for members to seek social support or vent their emotions. However, expressing certain specific experiences or emotions through text can be challenging for users independently. Using generative images has the potential to assist seekers in better self-disclosure. However, there is a lack of research on how to use generative images to assist seekers and how users perceive and use this technology. In this paper, we introduce a technical prototype called MentalImager, which can provide users with images related to the emotions and themes they want to express to assist them in self-disclosure. Results from a mixed-design methods study involving 24 participants indicate that MentalImager can generate images that meet users' requirements and inspire their writing. We report on the insights into MentalImager and suggest design considerations for image support in OMHCs.
\end{abstract}









==> sections/3_formative_study.tex <==
\section{Formative study}
% To gain a comprehensive understanding of the difficulties users face in self-disclosure of their mental health issues online and how generative images can assist them, we distributed a questionnaire to 34 individuals who had recently experienced negative emotions or disclosed negative emotions to others. 
\peng{
\subsection{Survey Protocol}
\begin{itemize}
    \item Please refer CriTrainer for the necessary details of the study: "We develop our questionnaire on Microsoft Forms and invite our respondents to fill it online. It first asks for respondents’ prior experience and perceived ability in critical paper reading. For those with experience in critical paper reading, we further ask about their encountered difficulties in critical paper reading practices when they were beginners in critical paper read- ing practices. To elicit novices’ needs for support in each training stage, we brainstorm a set of potential features (Table 1) of the training tool, based on their paper reading experience and related works (e.g., CReBot [65 ], Marvista [ 19 ], the theory of scaffolding [33 ]). We then ask participants to rate their perceived usefulness of these features on a standard five-point Likert scale (1 - not useful at all, 5 - very useful). We also include open-ended questions about other features they would like to have in the training support tool."
\end{itemize}
\subsection{Respondents}
\begin{itemize}
    \item Please refer to CriTrainer and MepsBot, move the PHQ-9 information, mental health issues to here
    \item MepsBot: "Previous research suggests that the majority of college students experience some forms of mental distress [8, 46, 63]. The self-assessments on the severity of depression (measure: PHQ-9 [45]) in pre- screening show that our participants could have at least moder- ate depression: seven moderate (score 10-14), 18 moderately severe (15-19), and five severe (20-27) [53]. The depress- ing issues they encountered are mostly about Ph.D. research (count: 15), relationships with boy/girlfriend or families (6), and future direction (4). Six of them report having experience in OMHCs, and all participants are very familiar with online communities."
    \item CriTrainer: "We recruited 52 students (S1-52; 18 Females, 29 Males, 4 Not to specify) through social networks and word-of- mouth. They all speak English as their second language. Among them were 30 undergraduate, 15 master, and 7 Ph.D. students. Their ages range from 18 to 28 years old with an average age of 23 (SD = 2.23). Twenty-five respondents reported having no or little knowl- edge, 18 respondents had moderate knowledge, and the rest 9 peo- ple know a lot about critical paper reading. Forty-nine students indicated prior experience in reading scientific papers."
\end{itemize}
\subsection{Findings}
\subsubsection{Practices and Challenges of Online Mental Health Self-Disclosure}
\begin{itemize}
    \item One paragraph could be enough, if we have ratings, numbers of participants who talk about it, and representative quotes, please report them. 
\end{itemize}
\subsubsection{Needs for Generated Images for Assisting Mental Health Self-Disclosure}
\begin{itemize}
    \item Consider that we only have ratings on three features, we can use bullet points (the table with three lines is not necessary). If we have ratings, numbers of participants who talk about it, and representative quotes, please report them. 
\end{itemize}
\subsection{Design Requirements for MentalImager}
\begin{itemize}
    \item For each of the two design requirements, please 1) clearly link it to the challenge and needs in the section above, and 2) add references to related work as well
\end{itemize}
}



\update{
To gain a comprehensive understanding of the difficulties users face when engaging in self-disclosure in online mental health communities and when expressing emotions through images, we distributed surveys at two local universities. Subsequently, we presented some features brainstormed by HCI experts for them to rate, aiming to explore what functionalities our assistant needs to assist them. These scores guided the design of our system's features. Additionally, we provided three sets of images generated by the model to investigate users' acceptance of generative images. Finally, we conducted random interviews with six individuals to delve into the specific reasons behind their ratings.
}
% This study revealed some difficulties users encounter when self-disclosure in the online community. It also provided further guidance for developing MentalImager to address their difficulties and needs in mental health self-disclosure.
    \subsection{Participants and Procedure}
    \subsubsection{survey research}
     We distributed the questionnaire to 34 students (14 males, 16 females, 4 prefer not to say, age: 19-24, SD=1.6) who have the experience of using online community for self-disclosure in two local universities. % in China using WenJuanXing\footnote{https://www.wjx.cn/}. 
     % In total, 34 participants were recruited for the formative study (14 males, 16 females,4 prefer not to say, age range 19-24, SD=1.6). Here's how we conducted the survey.
     The questionnaire starts with the Patient Health Questionnaire-9 (PHQ-9)\cite{phq9} to determine if users had experienced symptoms of depression in the past two weeks. 
     Then, it asked if users had experienced distress due to negative emotions and inquired about their desire for self-disclosure.
     % All of the participants had been troubled by negative emotions or experiences, or had recent depressive symptoms and had a desire for self-disclosure.
     % In the subsequent questionnaire survey, we asked
     Next, the questionnaire asks them about the difficulties they encountered when engaging in self-disclosure and why. 
     Then, it asks about their experiences of attaching images for mental health self-disclosure, the challenges they faced in doing so, and how they think the images could benefit their self-disclosure.
     \update{
     Users who encountered difficulties in using images were asked to rate the functionalities brainstormed by several HCI experts. They were also given the opportunity to suggest additional features they wished to have.

     \subsubsection{Interview}  We randomly selected 6(3 males, 3 females) participants from those willing to take part in further experiments and conducted 10-minute interviews. We inquired about how they overcame difficulties encountered while completing the questionnaire and their specific thoughts on using generative images to aid in self-disclosure.
     }
     

    \subsection{Findings}
    % In the survey, we found that X people agreed that using image-text would be more suitable for expressing these experiences or emotions, and X people believed that using images would assist them in better self-expression. However, some users couldn't find suitable images locally, and others could find the required images online but found it time-consuming.

    % Additionally, we found that users expressed a strong willingness to have the assistant quickly provide images related to their content and emotions. This influenced our choice of dimensions to investigate user image acceptance. Considering that generative images could sometimes produce incorrect images that users might find unacceptable, we also asked users to rate the visual appeal of the images. We found that, in user ratings, generative images did score slightly lower in quality compared to retrieval images. However, they scored higher in the other two dimensions, and overall, generative images received higher composite scores than retrieval-based ones. This demonstrates the users' higher acceptance of generative images. [ give data analysis and detials ]

    % ........[explaining survey data ]
    % The survey results indicate that most people believe that sharing images can help them express themselves, but they often encounter difficulties such as not finding suitable images, which hinders their ability to self-disclose effectively, and may even lead them to refrain from posting altogether. The survey results indicate that most people believe that sharing images can help them express themselves, but they often encounter difficulties such as not finding suitable images, which hinders their ability to self-disclose effectively, and may even lead them to refrain from posting altogether. We are considering the use of generative images to meet users' image needs, which can be more adaptive compared to grabbing or retrieval. Additionally, we need to consider how to engage users more in the image generation process to facilitate better self-disclosure. Additionally, we need to consider how to engage users more in the image generation process to facilitate better self-disclosure. Based on the reasons mentioned above, we propose the following two design requirements (DRs): 1. How can generative images assist users in self-disclosure? 2. How can generated images be made relevant to the emotions and themes of the users

    % In general, 14 participants mentioned experiencing stress related to their studies (e.g., graduate entrance exams and stress from exam weeks), seven related to dealing with social relationships (e.g., arguments with friends), five about their families (e.g., family emotional violence), and four about difficulties in dealing with romantic relationships (e.g., breakups). 
    % 25 participants mentioned that it was challenging to use plain text to describe their anxiety and pressure caused by topics like study or romantic relationships. 
    \update{
    In general, we derived insights into the challenges users face when using images for self-disclosure from the questionnaire and semi-structured interviews. Their expressed needs further guided our subsequent system functionality design and feasibility experiments.
    \subsubsection{Key-issue} participants mentioned many aspects they had difficulties in using images to express their emotions. For instance, studies (e.g., graduate entrance exams and stress from exam weeks), dealing with social relationships (e.g., arguments with friends), family (e.g., family emotional violence), deal with romantic relationships (e.g., breakups).In the interviews, we find that participants and those around them often choose to either edit the text to corresponding existing images or abandon this post when they can not find suitable images, and the main reason for doing this is to ensure alignment between their images and text. The scoring results from the questionnaire indicate that this alignment is generally related to thematic and emotional relevance. And the challenges users face in using images for self-disclosure often stem from: a lack of relevant local images, the inability to find suitable images online, and uncertainty about what images are appropriate to use.

    \subsubsection{Needs} 22 participants agreed that adding images to their posts helped them express themselves because they believed that images were more powerful than text in expressing these ambiguous emotions or experiences, which aligns with \cite{Manikonda17, Kaplan10}. However, this leads users to always want to enhance their posts with images to add emotion or make them more attractive. From the survey results, their main need is to always get the desired images even if they don't have them on their devices, which is reasonable. Among the features we provided, the highest scores were for providing images based on text topic and emotion, which is consistent with \cite{Zhao16}'s findings. We also noticed that some users want to further modify the generated images or be more involved in the image generation process. We found that this idea is somewhat similar to Art Therapy\cite{Nicki23} and should also be considered in our design.
    } 
    %, while including images in the posts had helped them. 
    % We found that 25 participants described the anxiety and pressure brought about by studying or the difficulties they encounter in romantic relationships are often challenging. Because text struggles to convey these abstract topics, or expressing them in the text is inherently difficult, this is also the reason why they include images to assist themselves express in their posts.
    % Additionally, 22 participants agreed that adding images to their posts helped them express themselves, as they believed that images were more powerful than text in expressing these ambiguous emotions or experiences. \textit{``When I express (the emotion of) failure, images can convey strong feelings more effectively''}. 
    % This phenomenon aligns with \cite{Manikonda17, Kaplan10}.
    
    % However, participants encountered various difficulties when selecting images for their posts.
    % 20 participants mentioned that they could not find suitable images on their devices at least once when they wanted to disclose their issues online. 
    % 14 participants reported that they often spend time searching online for suitable images. 
    % 19 participants went through moments of lacking inspiration for choosing images. 
    % In the survey, users expressed their desire for our tool to provide images based on their input content. They also wished for the provided images to be relevant to their topics and emotions, believing that such images would help them better express their needs or vent their emotions. Additionally, 19 users expressed a desire to be able to modify the provided images. \textit{``I wish to make further modifications to the provided images.''(S34)}
    
\update{
After we observe a strong willingness among users to use generative images to express their emotions, how to provide users with the images they need, ensuring that the content of generated images aligns with their text, and exploring their satisfaction with these generated images still requires further investigation. Based on the findings above, we giving: DR 1) Generate images related to user text content and emotions. DR 2) Allow users to modify images themselves.
}
    



==> sections/4_Feasibility_Exploration.tex <==
% \section{Design}
% \pzh{Note: If there are related findings (e.g., practices, challenges, needed support) from our previous survey study, we can have this subsection to summarize the design goal.
% If not, we have to find another way to describe how we come up with the design, e.g., fully theory-driven (this is tricky in the writing and is easily challenged by reviewers). 
% If we have this section, please refer to the CriTrainer paper for the writing. 
% }

% \zyx{
% In the initial stage of our study, we started with a survey aimed at understanding how images are used in online communities. 

% We gathered responses from 70 valid questionnaires, with 37 males and 33 females participating. 
% Notably, 36 respondents (51.43 \% ) shared that they have expressed negative emotions or content on social platforms.

% \begin{itemize}
%     \item There is a lack of photographic data here.
% \end{itemize}

% When it comes to expressing emotions, participants encountered challenges related to images, like finding it difficult to accurately describe their feelings in words struggling to find images that match their emotions, and experiencing uncertainty about what to express in the first place.

% Additionally, participants faced obstacles while using images to convey their emotions:
% In the questionnaire, a number of people said they have limited availability of appropriate local images, great difficulty finding suitable images online, or uncertainty about selecting images that truly communicate their emotions.

% Considering these challenges, we distilled three key research questions: 
% Research Question 1(RQ 1): How can images be effectively used to enhance users' emotional expression?
% Research Question 2a(RQ 2a): When using our image assistance tool, how can we ensure the suggested images match the context of user-generated content?
% Research Question 2b(RQ 2b): When using our image assistance tool, how can we ensure the suggested images align with users' emotional feelings?

% Within the functionalities we proposed, the image generation feature stood out with high ratings:

% 1. Users highly endorsed the recommendation of usable images based on emotional keywords(, giving it a score of 3.36 on a 5-point scale.

% 2. The suggestion of usable images based on thematic keywords received a score of 3.27, indicating significant support for this approach.

% 3. Evaluating the recommendation of images based on the entire content, the score reached 3.29, highlighting strong backing for content-based image recommendations.

% \begin{itemize}
%     \item There is a lack of photographic data here.
% \end{itemize}

% This analysis, combined with image rating records, formed the basis for outlining the following design requirements: 
% Design Requirements 1(DR 1): Incorporate generative images for adaptive image support.

% -Reason: The challenges faced by users in finding suitable images that resonate with their emotions highlight the need for a more adaptable solution.  
% Generative images, produced algorithmically, offer a promising approach.  
% These images can be tailored to closely match the user's emotional context, thus bridging the gap between the user's emotional expression and image availability.

% Design Requirements 2a(DR 2a): Utilize two distinct image generation methods to ensure relevance:

% (1)Keywords-based method: Extract keywords from titles to create topic tags.

% -Reason: The keywords-based method ensures that images are generated based on the specific themes communicated in the user's content.  
% Extracting keywords from titles and forming topic tags enhances the relevancy of the generated images.

% (2)Content-based method: Generate keywords based on the entire text content.

% -Reason: The content-based method tackles the challenge of contextual matching by generating images that correspond directly to the textual content, providing users with images that accurately capture their intended message.

% Design Requirements 2b(DR 2b): Extract emotional keywords from content for emotional relevance.

% -Reason: Emotional expression is a crucial aspect of image-based communication.  
% Extracting emotional keywords from the user's content ensures that the generated images align with the emotional sentiments they aim to convey.  
% This requirement addresses the issue of users struggling to find images that accurately reflect their emotions.  
% By considering emotional keywords, the generated images can effectively amplify the emotional impact of the user's content, resulting in a more authentic and meaningful expression.

% And then we will implement the tool we developed according to the design goals summarized above in the following.

% }
% Report the survey results
% \pzh{
% \begin{itemize}
%     \item Difficulties: general (including text) <-- how image may help (reference); about images <-- how generate images can help 
%     \item Rating on the features + difficulties + references --> propose the design requirements
% \end{itemize}
% }


\section{Feasibility of Generating Topic- and Emotion-Relevant Images of a Mental Health Support-Seeking Post}

% According to the results obtained from the formative study, users expressed a desire for images that are relevant to the content and emotions they want to convey in their posts.
\update{Given that we don't know how users evaluate the alignment between the model-generated images and the text,} in this section, we explored how to generate images that are related to the topic and emotions users want to express. 
We compared three textual prompts to the text-to-image generation model with a baseline approach that uses the Google Search engine to retrieve an existing image. 
We randomly sampled 20 posts from the Reddit r/depression community and used them to generate 60 (3 $\times$ 20) images and retrieve 20 images online.  
We invited the six raters who were interviewed in Section 3 to score the shuffled four images of each post from three aspects. 
\update{These three dimensions were designed to align with findings in Section 3:}
    \textbf{visual quality} (overall quality of the generated images), 
    \textbf{topic relevance} (the degree of relevance between the images generated and the topic content expressed in the respective posts), 
    and \textbf{emotion relevance} (The degree of relevance between the images generated and the emotional content expressed in the respective posts). 
    All items are rated on a 5-point Likert Scale, with 1 being the worst and 5 being the best.

% compared the results with images obtained from online searches. For image evaluation, we invited six raters (3 males and 3 females) to rate our images on three dimensions. We then used one-way ANOVA to analyze the dimensions and conducted post-hoc tests on the data. These results will guide our choice of text-to-image methods to be used in the system.

    \subsection{Retrieval-Based Baseline}\label{sec:TF-IDF}
    The baseline method retrieves the first returned image from the Google Image Search engine \footnote{https://images.google.com/} based on the extracted keywords from posts. 
    We implemented a traditional \textbf{keyword extraction approach} by using the nltk toolkit to tokenize the text of the content and title of a post, using the Rake function of nltk to extract keywords, and calculating the TF-IDF score for each extracted keyword. 
    We used the top five words from each post, in descending order based on their TF-IDF scores, to query Google Image Engine. 
    % We started by collecting 20 random historical posts from the r/depression subreddit and then considered generating images based on these 20 posts. We used every single historical post as a simulated user post to test image generation. We take both the title and content of the post as our input for analysis. 
    % First, we tokenized the text of the content and title using the nltk toolkit. 
    % Next, we used the TF-IDF method to construct a vocabulary matrix from the obtained words, thereby extracting keywords.
    % First, we tokenized the text of the content and title using the nltk toolkit, which forms the original documents. 
    % Next, we extract keywords from the text of content by the Rake function of nltk, then calculate the TF-IDF score for each word in the title. We then selected the top five words from each post, in descending order based on their TF-IDF scores, to use as query words.  
    % Next, we used the TF-IDF method to calculate the construct of a vocabulary matrix from the original documents, and selected posts' keywords based on [xxx].  
    % We then used these keywords to find images using Google Image Search\footnote{https://images.google.com/}, which is similar to how users search for images in their daily lives. 
    % Finally, we selected the first image returned by the Google search engine as the image used in the baseline system for comparison with images generated by the model. 
    % % We then used these keywords to find images using Google Image Search\footnote{https://images.google.com/} and took the first result returned as the image selected, which is similar to how users search for images in their daily lives [ref]. 
    % We input these keywords into Google search to find images. This method of image searching is similar to how users search for images in their daily lives. 
    % Therefore, we consider the first result returned as the image selected by the user and use it as the baseline for comparison with images generated by the model.
    % Considering that we need to investigate users' acceptance of the images generated by our model compared to real images.
    % For keywords extracted from the title, we are only interested in the most important word since we assume that a post typically revolves around a single topic. These title keywords will serve as topic tags.
    
    
    % Therefore, we use real images as a baseline for comparison: in the second method, the keywords obtained will also be input into Google Images search to search for images, and the first image returned will be used as the baseline.
    

    \subsection{Image Generation based on Three Types of Textual Prompts}
        \subsubsection{Model}
        We chose the anything-v5 pre-trained model \cite{Li23}, which is an open-source pre-trained Stable Diffusion model. It can generate images in animation style based on textual input and is widely used for non-commercial artistic creation. We opted for an animation style to mitigate the risk of the model inadvertently infringing on individuals' likeness rights or causing negative psychological experiences for users \cite{Berking12}, e.g., the ``uncanny valley'' effect \cite{Mori12}.

        \subsubsection{Textual prompts}
        % Given that our text-to-image model is based on Stable Diffusion, which supports two types of text inputs for image generation: keywords and sentences. 
        Our text-to-image model supports two types of textual inputs to generate images: keywords and sentences. 
        We \update{designed} three different textual prompts for the model to explore their advantages and disadvantages in generating images based on the mental health support-seeking posts, \update{which also received the highest user ratings in the questionnaire}:

        1) \textbf{Content-based}: the textual content of the posts. % directly as input to the model to generate images.

        2) \textbf{Basic keywords based}: the extracted keywords from the post's content using the TF-IDF method (similar to the baseline model without keywords in the title). %, which is input to the model to generate images.
    
        3) \textbf{Emotion- and topic- relevant}: the extracted keywords from the post's content using the TF-IDF method + additional keywords about the post's emotion + extracted keywords from the post's title.  
        %, we also extracted keywords from the post's title. Moreover, we also consider the emotion-related information since the support-seek posts in OMHCs should also be emotion-relevant.  
        We used a pre-trained BERT-based model \cite{Hartmann22} to determine the emotion conveyed in the post's content. It can categorize content into one of the seven basic emotions (\ie emotional keywords in our case): anger, disgust, fear, joy, neutral, sadness, and surprise. %The outputs of these three processes (i.e., keywords from post content and title, as well as the recognized emotion) were used as input to the model to generate images.

        \subsubsection{Processing the keyword-based prompts}
        % For inputs based on sentences, the CLIP layer of the model can independently assess the utility of each sentence in the text \cite{Li23}, so no additional actions are needed to avoid introducing more bias. However, for inputs based on keywords, since the model cannot independently judge the utility of each keyword, we need to ensure the input's utility as much as possible \cite{She20}.
Although our selected text-to-image model can take both sentences and keywords as input, the image generated based on keywords is often irrelevant to the topic as context information is lost in the extraction process~\cite{Li23, She20}.
\update{When generating images, synonymous substitutions for keywords do not significantly impact the content of the images\cite{Liu22}. However, for the model, this can reduce the probability of generating incorrect images\cite{Kurzhals23}.}
Reasonably, to ensure the utility of the extracted keywords, we designed a WordNet to remove irrelevant keywords from image generation, such as pronouns and auxiliary words. Additionally, this WordNet will be used for synonym conversion to ensure that the provided keywords are all understandable by the model.
% Additionally, for keywords-based image generation, we need to adjust the weights of keywords to influence the process of image generation. 
Then, for keywords-based image generation, we allow users to adjust the weights of keywords, which can change the generated image.  
We use the default initial weight ``1'' for each extracted keyword in the text-to-image generation model. %, which is also the default setting for the keywords-based input. 
For the additional emotional keywords and topic keywords, we adjust their default weight to ``1.3'' based on our trials to prompt the model to generate emotion- and topic- relevant images. 
% We want the model to focus on the emotion keyword and topic keyword, so their weights are initially adjusted to 1.3. 
Additionally, we also rank the nouns and adjectives in the content by importance matrix generated in \ref{sec:TF-IDF} and extract all of the top 5. If any of these words appear in extracted keywords, it will increase the weight of that keyword by 0.1.
    



\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{figures/post.png} 
  \caption{One of the posts used for user rating. The left side shows the post's title and content, while the right side displays the images obtained from the four methods: (a) image from Google images search, (b) content-based method, (c) without extra keywords method, and (d) with extra keywords method. The keywords of (c) are: \textit{broken,  happy, depressed, pity, displaying self pity, 0 self confidence, someone please get, said, works, understands}. For (d), in addition to all the keywords from (c), there are additional emotion keywords obtained through BERT analysis: \textit{sadness}, as well as topic keywords extracted from the title: \textit{hopeless}.
}
  \label{fig:post}
\end{figure}

    % \subsection{User rating}
    % We recruited 6 raters (3 males and 3 females, aged 19-22) through verbal invitations, all of whom had experience in accompanying images for posts. Each rater was tasked with evaluating 20 sets of images, each containing 4 pictures (3 generated and 1 retrieval). Considering the focus of our study, we asked the raters to score the images on three dimensions, ranging from 1 to 5 points, with 1 being the worst and 5 being the best. These three dimensions were:
    % \textbf{visual quality} (overall quality of the generated images), 
    % \textbf{topic relevance} (the degree of relevance between the images generated and the topic content expressed in the respective posts), 
    % and \textbf{emotion relevance} (The degree of relevance between the images generated and the emotional content expressed in the respective posts). 
    % It is worth noting that, considering that the order in which the images are presented can introduce bias, we ensured that, for each rater, the 4 images in each set were randomized during the scoring process to mitigate this potential error. In our ANOVA analysis, we found no significant differences in scoring between different orderings of images.
    



    \subsection{Findings}
    % We recruited six raters to score the four methods mentioned above on a scale ranging from 1 to 5. They considered the following aspects: 
    % 1) The degree of relevance between the images generated and the topic content expressed in the respective posts (topic relevance).
    % 2) The degree of relevance between the images generated and the emotional content expressed in the respective posts (emotion relevance).
    % Additionally, we sought to gauge user acceptance of generative images in comparison to real images. Therefore, raters were also required to consider 3)The overall quality of the generated images (visual quality).

We use the one-way repeated-measured ANOVA to assess the statistical differences among the four methods (one baseline method and three image-generation methods).  
As shown in Table \ref{tab:ANOVA}, we observe significant differences among the four methods regarding the metrics of visual quality, topic relevance, and emotion relevance ($p < 0.001$). 
    % The collected scores were subjected to statistical analysis utilizing the one-way ANOVA method and the Wilcoxon test ($P=0.05$) was used to assess the significance of the differences in their scores, with results presented in the table \ref{tab:ANOVA}. Statistically significant differences were observed evidently in the scores across the four methods ($w>0.05, p < 0.05$). 
    % It was noted that compared to the retrieval-based method (the baseline), all three kinds of images generated through the text-to-image model obtained higher scores in terms of topic relevance and emotion relevance, albeit exhibiting slightly lower visual quality. 
    Compared to the retrieval-based method (the baseline), all three generation-based methods obtained higher scores in terms of topic relevance and emotion relevance, albeit exhibiting slightly lower visual quality. 
    Furthermore, compared to other methods, the prompt with emotion- and topic- relevant demonstrated the best performance in generating topic- and emotion-relevance images.
    Therefore, we choose the emotion- and topic- relevant method as the default method to generate images in the later implementation of MentalImager. 
    
    % in scores across all three dimensions.
% However, due to the slightly lower visual quality of the generative images compared to real images, we asked each rater for their opinion on the visual quality of the generative images.
As the visual quality of the generative images is often slightly lower compared to real images, we asked each rater for their opinion on the quality of the generative images. 
All raters considered the quality of generative images acceptable for use. However, raters reported that the generated images tend to convey a lower sense of realism compared to images depicting the real world due to 
Because our model generates images in an animated style, it tends to convey a lower sense of realism compared to images depicting the real world. 
As one rater said \textit{``Real images look more like photographs, but generative images look more like drawings. Both of them are acceptable to me, but photographs give a higher sense of realism, so I gave a lower score to the generative images''(R1)}. However, generative images excel in conveying emotions compared to real images: \textbf{``I believe generative images are more relevant to the emotions or topic that the post wants to express (compared to real images). If it were me posting, I would prefer to choose images that are more relevant to the emotions or themes of my post.'' (R3)}

    % Notably, with extra keywords method yielded the highest mean value of emotional and topic relevance. Consequently, this method was selected to provide the text-to-image model with keyword input. In light of the commendable performance of the content-based method in the quality of image generation, we also selected this method to provide sentence input, thus affording users a broader range of choices.

% \begin{table}[h]
% \caption{Analysis of user ratings, and in the ``Method'' column, 1 represents the baseline method, 2 represents content-based method, 3 represents basic keywords based method, and 4 represents emotion- and topic- relevant method. \textit{w} represents the variance homogeneity test result, and \textit{p} indicates the significance in the ANOVA analysis, where the p-values ($*:p < .050, **:p < .010, ***:p < .001$) is reported.}
% \label{tab:ANOVA}
% \begin{tabular}{ccccc}
% \cline{3-4}
%                                    &        & \multicolumn{2}{c}{Static} &                      \\ \hline
% Factor                             & Method & Mean        & S.D.         & p                    \\ \hline
% \multirow{4}{*}{Visutal quality}   & 1      & 3.0670      & 0.46436      & \multirow{4}{*}{***} \\
%                                    & 2      & 2.6665      & 0.42962      &                      \\
%                                    & 3      & 2.4915      & 0.41308      &                      \\
%                                    & 4      & 2.6575      & 0.29820      &                      \\ \hline
% \multirow{4}{*}{Topic relevance}   & 1      & 2.1255      & 0.87277      & \multirow{4}{*}{***} \\
%                                    & 2      & 2.7585      & 0.75635      &                      \\
%                                    & 3      & 2.3915      & 0.71673      &                      \\
%                                    & 4      & 3.2575      & 0.72655      &                      \\ \hline
% \multirow{4}{*}{Emotion relevance} & 1      & 2.3755      & 0.96773      & \multirow{4}{*}{**}  \\
%                                    & 2      & 3.2165      & 0.89261      &                      \\
%                                    & 3      & 2.5915      & 0.98570      &                      \\
%                                    & 4      & 3.7500      & 0.65240      &                      \\ \hline
% \end{tabular}
% \end{table}
\begin{table}[h]
\caption{Analysis of user ratings, and in the ``Method'' column, 1 represents the baseline method, 2 represents the content-based method, 3 represents the basic keywords-based method, and 4 represents emotion- and topic- relevant method. \textit{w} represents the variance homogeneity test result, and \textit{p} indicates the significance in the ANOVA analysis, where the p-values ($*:p < .050, **:p < .010, ***:p < .001$) is reported.}
\label{tab:ANOVA}
\begin{tabular}{cccclc}
\cline{3-4}
                                   &        & \multicolumn{2}{c}{Static} &                        &                      \\ \hline
Factor                             & Method & Mean        & S.D.         & F                      & p                    \\ \hline
\multirow{4}{*}{Visutal quality}   & 1      & 3.0670      & 0.46436      & \multirow{4}{*}{7.251} & \multirow{4}{*}{***} \\
                                   & 2      & 2.6665      & 0.42962      &                        &                      \\
                                   & 3      & 2.4915      & 0.41308      &                        &                      \\
                                   & 4      & 2.6575      & 0.29820      &                        &                      \\ \hline
\multirow{4}{*}{Topic relevance}   & 1      & 2.1255      & 0.87277      & \multirow{4}{*}{8.101} & \multirow{4}{*}{***} \\
                                   & 2      & 2.7585      & 0.75635      &                        &                      \\
                                   & 3      & 2.3915      & 0.71673      &                        &                      \\
                                   & 4      & 3.2575      & 0.72655      &                        &                      \\ \hline
\multirow{4}{*}{Emotion relevance} & 1      & 2.3755      & 0.96773      & \multirow{4}{*}{9.925} & \multirow{4}{*}{**}  \\
                                   & 2      & 3.2165      & 0.89261      &                        &                      \\
                                   & 3      & 2.5915      & 0.98570      &                        &                      \\
                                   & 4      & 3.7500      & 0.65240      &                        &                      \\ \hline
\end{tabular}
\end{table}





% \begin{table}[h]
% \caption{The results of the Wilcoxon Signed Ranks Test, where B, v1, v2, v3 represent the visual quality rating of baseline, first method, second method, and third method}
% \begin{tabular}{lrrr}
% \hline
% \multicolumn{4}{c}{\textbf{Wilcoxon Signed Ranks Test}}                                                   \\ \hline
%                 & \multicolumn{1}{c}{v1 - B} & \multicolumn{1}{c}{v2 - B} & \multicolumn{1}{c}{v3 - B} \\ \hline
% Z               & -2.268b                     & -3.285b                     & -2.693b                     \\
% p (2-tailed) & 0.023                       & 0.001                       & 0.007                      \\ \hline
% \end{tabular}
% \label{tab:Wilcoxon}
% \end{table}




==> sections/5_system.tex <==
\section{\name{}'s Design Requirements and Interaction}

In this section, we present MentalImager, a prototype system designed to facilitate self-disclosure among users in OMHCs using generative images with their self-disclosure.
First, based on the survey findings and relevant literature, we formulated two design requirements (DRs) for MentalImager. 


% Note that we do not intend to position MentalImager as a typical self-disclosure enhancement technology. Instead, we see it as a tool to explore the impact of different modes of expression on self-disclosure among OMHC users. To make the tool more engaging and interactive, we've designed the system as a robot that assists.
% In the remaining parts of this chapter, we introduced our user interface design and the relevant technology used to generate images for users.
    % \subsection{Design Requirements}
    \textbf{DR1: MentalImager should provide topic- and emotion-relevant images based on the user's drafted post.} Based on the survey, most users require images to assist them in expressing emotions. Images are promising to help users express certain specific emotions (\eg those about encountered mental health issues) or need more effectively than plain text \cite{Manikonda17, Rich02, Harden08}. 
    % However, they often lack suitable images on their devices. Once users have appropriate images, they can engage in self-disclosure more accurately \cite{Martin11}.

    \textbf{DR2: MentalImager should allow users to modify images.} Drawing can help people organize their thoughts, especially when expressing emotions \cite{Belkofer14}, and it can also serve as a therapeutic tool for mental health \cite{Rich02}. %We are considering 
    Involving users in the image generation process could simulate the act of drawing, which also meets the users' needs for interactive image generation. 
    % This would require less artistic skill from users.
    % Considering that our research is situated in the context of mental health communities, which have specific characteristics, based on previous research, we have learned that the process of drawing helps individuals with self-disclosure and enhances their emotional expression \cite{Belkofer14}. Since most people do not possess advanced drawing skills, our design simulates the process of drawing by generating images.


    
% We, then provided an outline of the differences between the community with MentalImager and the Baseline, along with explanations on how users should interact with MentalImager. 
Note that we position MentalImager as a tool to facilitate users' self-disclosure of mental health concerns in online communities. 
Users do not necessarily attach the generated images to their posts nor re-edit their posts if they do not feel like doing so. 
With MentalImager, we aim to explore whether and how the generated images affect support-seekers' self-disclosure outcomes and experience in OMHCs.
    
    \subsection{User Interface and Interaction}
        \subsubsection{User Interface}
        To facilitate user engagement in the image generation process, we considered adopting a design philosophy similar to the Stable Diffusion WebUI. This involves visualizing the steps that influence image generation directly on the web page through interactive means. First, to create an atmosphere reminiscent of an online mental health community for evaluating MentalImager, we emulated the design of Reddit to simulate a virtual community. Figure \ref{fig:baseline1} depicts the simulated baseline community interface without MentalImager, and Figure \ref{fig: tool explain} shows the community interface with MentalImager.
        In line with the current trends of posting both texts and images in online communities, we enable users to attach images to their posts. %which is also one of our research objectives,
        The design in both communities is as follows: In the baseline community interface, users can search for images they desire on the Internet or select images from their local storage. After clicking "Choose File" (the boxed area in Fig. \ref{fig:baseline1}) to upload the image, they can click the submit button to post it along with their textual content. 
        In the community with MentalImager, after users input the title and content and the "Generate Image" button ({b1} of Figure \ref{fig: tool explain}) is clicked, MentalImager will appear at the right of the user input area, and they can obtain a set of images provided by MentalImager, which takes approximately 5-7 seconds. It is noticeable that in this experiment, the set of images provided by MentalImager always consists of four distinct images (Figure \ref{fig: tool explain}).
        
        \subsubsection{Interaction}
        % To provide images related to user emotions and themes, we utilized the methods selected in feasibility exploration.
        While the default way of image generation is based on the extracted and additional keywords of the post content (according to the evaluation results in Table \ref{tab:ANOVA}), we also offer an option for image generation based on the full post content. 
        Below the self-introduction box of MentalImager, there are two buttons. Clicking the ``Keywords-based'' button on the right will generate a new set of images based on the current keywords in the keyword area (whether or not the user has made modifications). %, which uses the with extra keywords method, as shown in Figure \ref{fig: tool explain}. 
        On the other hand, the ``Content-based'' button on the left allows users to obtain a set of images generated directly based on the current text in the post content area. %, which uses content-based method. 
        Users can view detailed explanations about each button by hovering their mouse on the button. 
        Newly generated images will always appear at the top of the assistant, while previously generated images are shifted downwards. Users can click on the image with the left mouse button to zoom in and right-click to select images and include them when posting.
    
        In consideration of the pivotal role that keywords play in guiding users during the writing \cite{Shin22}, which helps users in organizing their language and writing thoughts. We have implemented a keyword section beneath the user input area. This section will exhibit all the keywords employed for image generation, each presented in a tag format as ``keyword: weight.'' Here, 'keyword' represents the comprehensive factors employed in the text-to-image model input, while 'weight' signifies the degree of significance assigned to the corresponding keyword during the image generation process. These tags are fully editable. Users can directly modify keywords through interactive clicks and adjust the weight using the provided plus and minus buttons. Moreover, users can exercise the option to either eliminate redundant tags or introduce new ones that align with their specific requisites.
        When adjusting tags, similar to the methods mentioned in \cite{Shin22}. Given that both content and keywords are editable, we adopt this approach to encourage users to generate images based on their ideas, mimicking the process of drawing in art therapy without requiring any artistic background \cite{Belkofer14}.
    

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/baseline1_1.png} 
  \caption{Baseline user interface. The appearance is designed to resemble the r/depression community to create an authentic community atmosphere. Users can upload local images by clicking the button inside the red box. The button text is in Chinese instead of English because the corresponding browser will change the language displayed for controls based on the user's country. After users input the title and content, they can click the Submit button to publish.}
  \label{fig:baseline1}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{figures/MentalImager_interface.png} 
  \caption{
  Screenshot of the MentalImager embedded in a simulated community. 
  %\textbf{(b1)} The button used to generate the initial image, which will be replaced later by \textit{(b2), (b3)}, \textbf{(b2)} Submission button, \textbf{(b3)}button that allows users to edit the text content. \textbf{(a)}MentalImager appears to the right of the posting area, with its self-introduction at the top of (a). Below the self-introduction are the two text-to-image methods we offer: \textbf{(d)}content-based and \textbf{(e)}keywords-based. \textbf{(f)}When users hover over these two buttons, corresponding function descriptions appear. \textbf{(c)}MentalImager also presents the keywords used for image generation in the form of tags below the user input area.
  }
  \label{fig: tool explain}
\end{figure}

    
    
    % \subsection{Text-to-image Generation}
    %     \subsubsection{Models}Talk about the three approaches
    %     Considering that Stable Diffusion (SD) \cite{Wu23, Kurzhals23} can accept two types of inputs: keyword-based and text-based, using text as input simply involves using the user's content as the input. However, based on our formative study, we recognized that users require images that are relevant to their emotions and themes. Therefore, we devised the following three methods to generate images by better extracting keywords from the user's text input:

    %     1. Using the entire user input text as the input for SD.
        
    %     2. Extracting keywords from the user's input text and using them as input.
        
    %     3. Extracting keywords from the user's input text, simultaneously analyzing the emotional content within the text, and incorporating information from the post's title.
        
    %     To assess the effectiveness of these three methods, we crawled 20 historical posts from Reddit's r/depression subreddit. For each post, we created 20 sets of examples, each consisting of the post's title, content, and four images. Three images were generated using the methods mentioned above, while the fourth image was obtained through web retrieval. We enlisted the participation of six users to rate these 20 sets of examples. The results indicate...
        

        % \zyx{
        % After conducting thorough research, we have identified three distinct methods for generating images from text and analyzed their respective advantages and disadvantages. These methods are:
        
        % 1. Generating Images through Keywords:
        % This technique involves creating images based on specific keywords provided as input. The system uses these keywords to construct visual representations corresponding to the given text. 
        % This approach gives users greater control over the generated images by allowing them to specify their desired visual elements. 
        % However, its effectiveness may be limited by the availability and diversity of image data associated with the provided keywords.
        
        % 2. Generating Images from Text:
        % In this method, the system generates images based on comprehensive textual descriptions or prompts. 
        % The advantage of this approach is its capacity for producing more detailed and nuanced image outputs, as it considers a broader contextual framework. 
        % Nevertheless, accurately capturing the desired visual elements solely from text can prove challenging, particularly when the descriptions are intricate or abstract.
        
        % 3. Searching for Desired Images on the Internet:
        % This method involves the retrieval of existing images from the internet, guided by the provided text. 
        % The primary advantage lies in its utilization of the vast reservoir of online image data, offering a wide array of image options. 
        % However, it relies heavily on the accessibility and relevance of online images, and it necessitates consideration of copyright and licensing factors when incorporating externally sourced images.
        
        % We plan to include questions in the user survey questionnaire to gather users' perceptions of these three text-to-image generation methods, followed by an analysis and comparison.
        % }
        
        % \subsubsection{Evaluation} @Yuxiang and @Han, Talk about the evaluation study, refer to the shared RetAssist VLS paper section 4.3.2 \textbf{(under submission, do not distribute it)}
        
            
        % \zyx{
        % We have implemented a comprehensive evaluation approach to assess the effectiveness of our experimental model. 
        % This approach involves gathering user feedback through interviews and surveys, covering various crucial aspects essential for comprehending the model's performance.
        
        % Our system's primary objectives revolve around several key aspects, including enhancing emotional expression through system-generated images, empowering users to seek psychological support and articulate their needs within the community, and ensuring that posts assisted by our writing tool are perceived as superior in conveying user emotions compared to those without assistance, and maintaining a seamless alignment between generated images and accompanying text.
        
        % User experience is of utmost importance, and we have distilled it into five key dimensions based on survey findings: enjoyment, convenience, workload, robustness, and practicality. 
        % The system should provide users with an enjoyable journey, offering an intuitive and user-friendly interface that prevents users from feeling overwhelmed or rushed. 
        % Any issues encountered during system usage should be manageable. 
        % The evaluation of practicality hinges on factors such as the consistency of generated keywords with user-intended emotional expressions, the effectiveness of generated images in facilitating users in seeking help and expressing emotions, and the overall empowerment of users within the psychological community.
        
        % Following this, we proceed to evaluate the system itself. 
        % System evaluation is a pivotal component, encompassing usability assessment and tool performance evaluation. 
        % Three crucial metrics—usefulness, ease of use, and intention to use—have been selected for in-depth analysis.
        
        % Useful for self-disclosure: Incorporating a measure of perceived usefulness aids in comprehending the tool or product's value and benefits to users, shedding light on whether the tool meets user needs and provides meaningful assistance in specific contexts.
        
        % Ease of use: The assessment of ease of use enables us to gauge the tool's user-friendliness and accessibility. 
        % This aspect determines whether the tool is intuitive, easy to navigate, and comprehend—a vital element for encouraging user adoption and satisfaction.
        
        % Intention to use: Measuring users' intention to use helps predict their willingness and likelihood to utilize the tool in the future, providing insights into user acceptance and potential long-term usage, thereby predicting the tool's success and sustainability.
        
        % The evaluation of the rationality of generated images aligns with the overarching goals of the system, ensuring that the generated images effectively contribute to user expression. 
        % The system should offer a seamless experience for both novice and experienced users, providing clear and logically sound feedback without imposing excessive cognitive effort or time constraints. 
        % The tool should enhance users' willingness to engage within the psychological community, and observers should find posts with assistant-generated content more comprehensible and engaging.
        
        % In conclusion, we seek impartial evaluations by soliciting blind ratings from external individuals. 
        % Our expectation was that these raters should show higher sensitivity to sentiment or need in Assistant-assisted posts, perceive a stronger correlation between text and images, and be more willing to respond to Assistant-assisted posts. 
        % Our multi-faceted evaluation process ensures a comprehensive understanding of our innovative system's performance, fostering continuous improvement and offering a valuable tool for enhanced emotional expression and psychological support within online communities.
        
        % }

    
 % keyword extract -> topic consistance
% emotion analysis -> emotion consistance

% keyword specific + emotion confirm -> tag
% tag -> stable diffusion(model) -> generate image
    

    % \subsection{Conception}
    % In this section, we will introduce an assistant prototype built within the OMHCs. This prototype will be utilized to aid newcomers (or those who have recently joined) in assisting with posting. Addressing the issues mentioned in the previous section, we will delve into the following discussions:
    % RQ1 Assisting users in expressing themselves accurately without violating community guidelines.
    % RQ2 Maintaining coherence with the accompanying text while utilizing generative images to aid users in expressing unique experiences or emotions.
    % RQ3 Does the use of generative images help posters express their needs more effectively and more accurately?
    % Therefore, we have decided to design a robot to implement these functionalities. In the process of implementing these functions, Feature 1) emotion and Feature 2) topic will play a crucial role.
    % \subsection{System Prototype of Assistant}
    % \subsubsection{\textit{Writing assistant}}Firstly, users are free to input the content they wish to post in the community, just as it would happen in real-life scenarios. The robot will automatically analyze the user's input to determine if the text violates any community rules. Additionally, by leveraging previously published posts within the community, the robot will provide users with recommended text modifications that align with the community's writing style. It is essential to note that the robot's suggestions are advisory rather than obligatory, aiming to avoid user frustration or aversion[].
    
    % As the writing conventions tend to be relatively stable within the same community[13], and the robot considers previously published posts within the community, the provided suggestions can ensure coherence with the community's writing style. During the process of offering recommendations, the robot will take into account the thematic ideas and emotions the user intends to convey. It will propose modifications that preserve the user's intended themes and emotions, thus ensuring the accuracy of the user's textual expression.
    
    % \subsubsection{\textit{Image assistant}}After analyzing the user's input emotions and topics, the robot will generate some images for the user based on these emotions and themes. In real-life situations, users typically use locally uploaded images in their posts, which allows the images to align with their expressive needs. However, image selection is highly subjective [34], meaning different individuals may have different feelings towards the same image. Therefore, employing a retrieval-based approach to recommend images from existing libraries may struggle to meet the users' specific requirements.
    
    % On the contrary, using a generative approach to create images based on the emotions and themes contained in the user's input ensures a strong connection between the recommended images and the user's text, thereby enhancing the likelihood of meeting the user's needs to a certain extent. Users are allowed to generate images multiple times, which enables them to regenerate images after modifying their text. Additionally, this feature takes into consideration that users may alter their text content based on the images we provide [20]. The objective is to ensure that the generated images remain aligned with the user's real-time input.




==> sections/6_experiment.tex <==
\section{Experiment}
To investigate MentalImager’s impact on support seekers’ experience in the self-disclosure process 
of mental health and the outcome of that process, we conducted a within-subject study with 24 participants. % and interviewed them.

\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{figures/task flow.png} 
  \caption{Research procedure of our study. 24 participants were randomly assigned to two groups that experienced the MentalImager and baseline interface in a different order.} % and used our/control interfaces, followed by the post, survey and interview sessions.}
  \label{fig: tool explain}
\end{figure}

    \subsection{Participants}
    During the pre-screening, we informed participants that the experiment would involve personal negative emotions or experiences. 
    We only include the participants who reported encountering mentally challenging issues within one month and indicated willingness ( > 4 on a 7-point Likert Scale, 1 - not willing at all, 7 - highly willing) to self-disclosure in online mental health communities. 
    We finally include 24 participants (P1-24, xxx males, xxx females, age: xxx-xxx) after screening the first 51 respondents to our recruitment survey distributed on social media. 
    % Subsequently, we identified users who had experienced or expressed negative emotions to others or in other ways in the recent past (within one month) and were willing to engage in self-disclosure in an online community. 
    % We finally recruited 26 participants (24 available, 2 Not Available) through a questionnaire-based recruitment process. The selection criteria required participants to have recent tendencies towards depression and a willingness to express their emotions or seek help through posting in an online community. 
    All participants were undergraduate students or currently pursuing an undergraduate degree with fluent English reading and writing abilities. 
    Participants' self-assessment on the Patient Health Questionnaire-9 (PHQ-9) \cite{phq9} indicated that they were at least classified as mild depression sufferers (scores between 5-9): 8 had moderate depression (scores between 10-14), and 5 had severe depression (scores between 15-27). 
    Their challenging experiences or emotions were mostly related to study and daily life. 
    For example, they reported stress associated with exam preparation, anxiety about not achieving the expected learning outcomes, irregular daily routines, and a lack of interest in daily life matters.
    To mitigate the order effect, we randomly assigned the participants into two equal-size groups (G1 and G2) that use the MentalImager and baseline interfaces in a different order (\autoref{fig: tool explain}). 
    % in the experiment were randomly assigned to one of two groups: one that used the assistant first or one that first tried the original community interface. This random assignment was done to mitigate any sequence-related biases.

    \subsection{Task and Procedure}
    
    % To evaluate the effectiveness of MentalImager, we defined two timestamps within the task:

    % \textbf{Pre-Image:} For the original community, this was before selecting a local image. For the community with MentalImager, this was before the user generated an image for the first time.

    % \textbf{Post-Image:} For the original community, this was before selecting the final content for posting. For the community with MentalImager, this was also before the user finalized their post.

    % To compare MentalImager with the existing mental health community environment, we designed a control interface. The key difference between the control system and our system was that the control system only allowed users to upload local images, while our system enabled users to use generative images. Other than this, their functionalities were identical. We conducted a within-subject study, where 12 participants were randomly assigned to consecutively use the control system and then our system, while another group used the reverse order. The research process is illustrated in the figure above.
Participants followed the experiment instructions in a document and used their computers to conduct the study remotely. 
They had two self-disclosure tasks. 
In each task, they first need to create a post in either the MentalImager or baseline interface to disclose their experience, thoughts, and feelings about a mentally challenging issue they recently faced. 
After each task, they need to fill in a questionnaire about their perception of the posting process and outcome as well as perception towards the interface. 
Upon completion of two tasks, participants informed the experimenter, who conducted a brief interview with each of them to learn more about whether and how the generated images could help mental health self-disclosure. 
Each participant received 27 RMB (\~ 4 USD) for about half an hour spent in the study. 
  
% Participants were required to 1) Choose a recent negative experience or emotion and write two posts. 2)Fill out a usability survey corresponding to each system after each post. 3) Participate in our usability survey and a brief interview at the end. Participants received a 27 RMB (approximately 4 USD) compensation at the end of the experiment, and research procedure of our study. 10 participants were randomly assigned to two conditions and used our/control interfaces, followed by the survey and interview sessions. We presented participants with sample posts from the r/depression community (with sensitive information removed) as examples. Data from all participants were not used for other participants' research.


    % \subsection{User Survey and Interview}
    
    % After each participant completed a post, we utilized a 7-point Likert scale (1 being strongly disagreed, 7 being strongly agreed), following literature \cite{Wu19}, to measure user usability and the level of assistance provided by MentalImager. As we needed to investigate the extent to which generative images helped users (DR 1), we considered asking the following questions regarding practicality (useful for self-disclosure): (i)Did the generated images effectively help the poster seek assistance or express emotions better? (ii)Did the assistant's provided images offer additional inspiration for my writing, or make my expression clearer?
    
    % After 24 participants completed their posts, we invited X users with experience in online mental health communities (OMHC) to blind-rate their posts, with all sensitive data removed. Given that we needed to study whether users wrote more empathetic and appealing posts (DR 2), we asked the raters to assess from four dimensions:
    % (i)Could you better sense the emotions or needs in the posts with the assistant's help (more empathy)?
    % (ii)Did you believe the textual content of the posts is consistent with the images in terms of emotion and theme(consistency of text and images)?
    % (iii)Were you more inclined to respond to posts with the assistant's help (more pleasure to reply)?
    
    \subsection{Measurement}
\subsubsection{Self-disclosure outcome} 
We capture how the generated images of MentalImager impact the self-disclosure in the posts from the aspects of both support-seekers and support-providers. 
In the questionnaire after each task, participants rated their perceived satisfaction of self-disclosure in their posts (\ie ``My mental health disclosure in the post is clear, and I am satisfied with it'') in a 7-point Likert Scale; 1 - strongly disagree, 7 - strongly agree. 
Upon completion of all studies, we invited another six people (3 males, 3 females, age: 20-22) who had experience in posting or commenting on online mental health communities to act as the support-providers. 
These six support-providers gave scores (1 - the lowest, 7 - the highest) on each of the shuffled support-seeking posts from our participants regarding: 

\begin{itemize}
    \item Degree of Empathy: To what extent can you sense the emotions or needs of the poster in this post? 
    \item Image-Text Relevance: Do you think the images in the post are relevant to the theme and emotions in the text?
    \item Willingness to Reply: Would you be willing to provide support or reply to this post?
\end{itemize}

We average the scores of the six raters on each dimension as the final score on that dimension for each post. 
The metric about the image-text relevance is only applicable to the posts that attach an image. 
    

\subsubsection{Self-disclosure experience}
In the questionnaire after each task, participants rated their perceived difficulty in disclosing their mental health experience, thoughts, and feelings; 1 - very easy, 7 - very difficult. 
If participants attached an image to their submitted post in the task with either MentalImager or baseline interface, we asked them to rate their perceived topic-relevance and emotion-relevance between the image and text of the post; 1 - least relevant, 7 - most relevant. 
If they did not attach an image, we asked them to give their reasons if any. 

    % We have implemented a comprehensive evaluation approach to assess the effectiveness of our experimental model. 
    % This approach involves gathering user feedback through interviews and surveys, covering two main aspects essential for comprehending the model's performance: usability and functionality. Additionally, to gain insight into how others perceive user posts, we incorporated a blind rating component.

\subsubsection{Perceptions towards MentalImager}
In the questionnaire after the task with MentalImager, we asked participants to rate its , the usefulness of its generated images for facilitating self-disclosure (four items), easiness to use (four items), adapted from \cite{Peng20}), and intention to use (two items), adapted from \cite{Wambsganss20, Peng20} as shown in \autoref{tab: evaluation}.

    % \textbf{Usability.} For the assessment of usability, to measure the usability of MentalImager for users we designed three dimensions \cite{Venkatesh08, Wambsganss20}.
    
    % \textbf{1) Useful for self-disclosure:} Incorporating a measure of perceived usefulness aids in comprehending the tool or product's value and benefits to users, shedding light on whether the tool meets user needs and provides meaningful assistance in specific contexts.
    
    % \textbf{2) Ease of use:} The assessment of ease of use enables us to gauge the tool's user-friendliness and accessibility. This aspect determines whether the tool is intuitive, easy to navigate, and comprehend—a vital element for encouraging user adoption and satisfaction.
    
    % \textbf{3) Intention to use:} Measuring users' intention to use helps predict their willingness and likelihood to utilize the tool in the future, providing insights into user acceptance and potential long-term usage, thereby predicting the tool's success and sustainability.
    
    % \textbf{Functionality} Similarly, to measure the tool's reasonableness in generating images, we considered three dimensions in total: 
    % 1) The relevance of the generated images to the post's content.
    
    % 2) The alignment of the generated images with the emotions the poster intended to convey. 
    
    % 3) The extent to which generative images aided in self-disclosure.

    % The design of these three dimensions aligns with user needs. We aim for users to receive images that are consistently relevant to the post's topic and preferably aligned with the user's emotions. Additionally, we require users to rate the inspiration they derive from the images to facilitate our analysis.

    \subsection{Ethical Concerns and Privacy Security}
    Our study protocol requires participants to describe their emotional status and background. The survey in both formative study and user study also includes some privacy-related questions (e.g., gender and experiences that make participants feel discouraged). Our user study requires participants to describe their emotions and background. 
    % , and the questionnaire includes some privacy-related questions (such as gender and negative experiences). 
    To protect participants' privacy, we have implemented and adhered to the following measures: (i) Our research has obtained university IRB approval, and we strictly follow the approved procedures; 
    (ii) All user transcript information is anonymized (e.g., using numbers to represent participants' names and schools) after collection; 
    (iii) Throughout the experiment, we adhere to the principle of voluntariness, we allow users to opt out of the experiment at any time they want. 
    (iv) For all participants in the study, we continue to monitor their mental status for one week.


% \begin{table}[h]
% \caption{Wilcoxon Significance test of posting with and without MentalImager assistance by users.}
% \begin{tabular}{lr}
% \multicolumn{2}{c}{\textbf{Wilcoxon Signed Rank Test Summary}} \\ \hline
% Total N                                             & 24                         \\ \hline
% Test   Statistic                                    & 4.000                      \\ \hline
% Standard   Error                                    & 14.040                     \\ \hline
% Standardized   Test Statistic                       & -2.956                     \\ \hline
% Asymptotic   Sig.(2-sided test)                     & 0.003                      \\ \hline
% \end{tabular}
% \end{table}




==> sections/7_discussion.tex <==
\section{Discussion}
In this work, we explore the feasibility, design, and impact of generated images to facilitate support-seekers' self-disclosure in online mental health communities. % have elucidated the viability of generative images in supporting self-disclosure within OMHCs and their potential to stimulate writing. 
% Specifically, based on our experimental results, 
Results from our experiments show that users can leverage generative images to satisfy their expressive needs in disclosing mentally challenging experiences, thoughts, and feelings. 
% across various contexts, with $Mean=3.25$ in topic relevance and $Mean=3.75$ in emotion relevance. While Baseline has $Mean=2.12$ in topic relevance and $Mean=2.37$ in emotion relevance. 
% At the same time, it also demonstrated the significant assistance of images in helping with self-disclosure in mental health, which aligns with previous work \cite{Rich02, Kaplan10, Manikonda17}.
These findings extend previous work on images for self-disclosure \cite{Rich02, Kaplan10, Manikonda17} by providing empirical evidence on the benefits of generative images to facilitate self-disclosure of mental health issues. 
We also found that support-providers can significantly better understand the support-seekers' feelings via the posts created with MentalImager and have a higher willingness to support them. 
This indicates that generative images can enable clearer self-disclosure and hold the potential to elicit a greater number of responses, which aligns with \cite{Luo20}. % as they are more capable of self-disclosure, which aligns with \cite{Luo20}. 
Besides, posts that exhibit a high degree of consistency between the text and generated images in terms of emotion and topic, which were created using generative images, tend to attract more responses, thereby increasing the satisfaction of the support-seekers \cite{Peng21}. 
We also have qualitative user feedback that involving users in the image generation process can facilitate superior articulation of their thoughts that art therapy encourages. % thereby amplifying their self-disclosure levels ($Mean=5.54, SD=1.28$). 
However, whether and how this interactive text-to-image generation approach can contribute to art therapy remains to be studied and proven.

% Furthermore, we have discerned that posts incorporating images are more apt to arouse interest among support-providers and elicit empathetic responses from them. 
However, we found that participants with MentalImager raised concerns about the style and quality of the generated images as well as the keyword extraction results. 
To address these concerns about using generated images to facilitate mental health self-disclosure, we provide the following design considerations. 
% Considering this constitutes a pivotal factor in nurturing robust online communities \cite{Kushner20}, we proffer the following salient considerations for system designers intending to deploy analogous systems in other OMHCs. 

% \ipstart{\textbf{Style diversity}}
\ipstart{\textbf{Providing style diversity}} If designers intend to promote similar systems to a larger and more diverse audience, we recommend considering the preparation of multiple text-to-image models with different styles within the system. This can enable users to choose the style of generative images according to their preferences or needs when self-disclosing different emotions. Additionally, designers should be cautious, as our experiments indicate that some negative inputs (e.g., depression) can produce imagery that induces negative and emotionally upsetting reactions when viewed~\cite{Berking12}. Therefore, designers should contemplate appropriate methods across styles to mitigate the generation of harmful or upsetting imagery, given the possibility of negative disclosures in OMHCs.  Such methods might recommend positive or neutral styles to accompany a user's negative input content (e.g., appending style-based keywords such as "light", and "pastel colors" upon detecting negative sentiment in the text), or detect and hide disturbing imagery by default and allow users to reveal them after a content warning.
% For example, appending style-based keywords such as "light", "pastel colors" upon detecting negative sentiment can create imagery where the styles are neutral or positive, while retaining the content of the mental health disclosure.    

% \ipstart{\textbf{Accurate extraction}}
\ipstart{\textbf{Context extraction with high accuracy}} Our survey reveals that users commonly engage in self-disclosure involving multiple topics. Expressing oneself with multi-topic content is challenging for individuals \cite{Peng19}, and understandably, we believe it's even more challenging for models. Designers should contemplate how to extract keywords from users when they are dealing with multi-topic content. For instance, employing classification algorithms to categorize users' keywords and building a keyword network could facilitate the model in making keyword associations across different topics.
% \subsection{Design Considerations}




% \subsection{Limitation and Future Work}

Our work has several limitations. First, We only explored the impact of generative images on helping users express negative experiences or emotions and did not investigate their role in facilitating positive emotional expression. 
Second, most of our participants are university students, which could not represent other specialized groups (such as pregnant women \cite{Gui17}). 
This confines our post topics to those pertinent to students, and the system's performance in more diverse or specialized contexts remains an unknown variable. 
Third, we measure the self-disclosure outcome from the support-providers' perspectives regarding their empathy with the support-seekers and willingness to offer support. 
It needs further explorations on how support-providers in a real online mental health community would perceive and reply to the posts created with the help of generated images. 
% notwithstanding our demonstrated enhancement of provider empathy through generative image utilization, the nuances of their interactions warrant further investigation. 
% Exploring the use of generative images as a mental therapy approach is also a direction we need to explore in the future.

\update{
In this work, We learned about users' thoughts on using generative images to help them self-disclose and designed a system based on their needs.


\subsection{Findings in generative image}
Results from our experiments show that users can leverage generative images to satisfy their expressive needs in disclosing mentally challenging experiences, thoughts, and feelings. 
We also found that support-providers can significantly better understand the support-seekers' feelings via the posts created with MentalImager and have a higher willingness to support them. 
This indicates that generative images can enable clearer self-disclosure and hold the potential to elicit a greater number of responses, which aligns with \cite{Luo20}.
\subsection{limitation}

\subsection{future work}
}




==> sections/7_result.tex <==
\section{Results}

We use one-way repeated-measured ANOVA to analyze the statistical difference between our MentalImager and baseline interface regarding the self-disclosure outcome and experience. 
For the qualitative user feedback in the interview, we code the transcript texts and group the codes into several themes, which are incorporated into the presentation of the results below. 
% For each ANOVA, the assumption of equal variance is confirmed by the Macuchly’s test of sphericity. 
% Before conducting the analysis, we performed a mixed ANOVA to assess the impact of the order of system exposure on the results and found that the order did not have a significant effect on the outcomes (\textbf{RQ 2}). Therefore, in the subsequent analyses, we used MentalImager as the sole independent variable. Additionally, based on the results of user interviews, we identified some concerns that should be taken into account when designing similar systems in the future.


\subsection{Self-disclosure outcome} 
As shown in Table \ref{tab:7-1}, support-seekers felt significantly more satisfied with their self-disclosure ($p < 0.05$) when creating the post with MentalImager than with the baseline interface. 
Our support-providers also reported a significantly higher degree of empathy with the emotions or needs of the support-seekers ($p < 0.001$) via the posts created in MentalImager than those in the baseline interface. 
They expressed a significantly higher willingness to reply to the posts created in MentalImager and provide support ($p < 0.001$). 
There is no significant difference regarding the perceived topic- and emotion-relevance of the text-image posts created in MentalImager and baseline interface ($p > 0.05$). 
This suggests that from the provider's perspective, the use of generative images does not result in weaker image-text relevance compared to real images, even though seekers may select images they perceive as more relevant. 
Additionally, considering that MentalImager should provide users with the images that users need rather than images that match more closely in emotion or topic, it is acceptable that there was no significant improvement in image-text relevance.

    \begin{table}[h]
    \caption{Means and standard deviation of the measurements on self-disclosure outcome and experience with Baseline and MentalImager.$ *:p < .050, **:p < .010, ***:p < .001$.}
    \label{tab:7-1}
    \begin{tabular}{ccccc}
\cline{3-4}
\multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                                                      & \multicolumn{2}{c}{Static}                                                                                                      & \multicolumn{1}{l}{} \\ \hline
Category                                    & Factor                                                                    & \begin{tabular}[c]{@{}c@{}}Baseline\\ Mean/S.D.\end{tabular} & \begin{tabular}[c]{@{}c@{}}MentalImager\\ Mean/S.D.\end{tabular} & P                    \\ \hline
\multirow{4}{*}{Self-disclosure Outcome}    & \begin{tabular}[c]{@{}c@{}}Satisfaction of\\ self-disclosure\end{tabular} & 4.67/.868                                                    & 5.54/0.72                                                        & ***                  \\
                                            & Empathy                                                                   & 4.26/1.37                                                    & 5.22/1.48                                                        & ***                  \\
                                            & Image-text relevance                                                      & 4.20/1.64                                                    & 4.21/1.57                                                        & 0.44                 \\
                                            & Willingness to reply                                                      & 3.63/1.53                                                    & 4.74/1.57                                                        & ***                  \\ \hline
\multirow{3}{*}{Self-disclosure Experience} & \begin{tabular}[c]{@{}c@{}}Difficulty in\\ self-disclosure\end{tabular}    & 4.58/1.248                                                   & 5.38/1.10                                                        & *                    \\
                                            & Emotion relevance                                                         & 4.12/1.72                                                    & 5.20/1.35                                                        & *                    \\
                                            & Topic relevance                                                           & 3.91/1.28                                                    & 5.45/1.21                                                        & ***                  \\ \hline
\end{tabular}
    \end{table}

\subsection{Self-disclosure experience}
In general (Table \ref{tab:7-1}), participants felt that compared to the baseline interface, it was easier for them to disclose their mental health concerns and feelings in MentalImager ($p > 0.05$). 
In total, all participants attach an image in their posts created with MentalImager, while the number in the baseline condition is 13. 
When they created text-image posts, they felt that the topic-relevance ($p < 0.05$) and emotion-relevance ($p < 0.05$) between the image and text were significantly higher in the posts created in MentalImager than those in the baseline interface. 
In the interview, 23 participants mentioned that they have a better experience in mental health self-disclosure with MentalImager's generated images. 
We identified two main themes about how MentalImager helped the participants.


    \textbf{Expression in text}. Fourteen participants reported that they received inspiration from the generated images and during the process of editing keywords to regenerate the images. For example, P10 stated, ``I wanted to express the struggle at the time when I was confused about my future. However, I did not know how to describe the feeling. When I saw a generated image in which a person stands on top of a mountain, it reminded me of the feeling that I was striving for my dream. Whenever I feel like giving up, it is my original dream that helps me move on''.
    % Consequently, the participant wrote, \textit{``Whenever I feel like giving up, I always think of the original dream.''} 
    P13 mentioned how he modified the wordings in the post when interacting with the generated images: ``When describing the pain caused by the pressure of my study, I initially used 'stressful'. However, during the process of adjusting the keywords to regenerate images, I found an image in which a girl curls up in a corner, which made me think of a 'bottomless pit' (representing endless stress).'' 
    Consequently, P13 changed the post's title from \textit{Stressful} to \textit{Tremendous pressure of study} and wrote, \textit{``I feel trapped in a bottomless pit of learning''}.
    We also found that modifying keywords for regenerating images could also be inspiring, which aligns with previous research in 
    % \qingyu{mental health communities}
    \cite{Shin22}. For example, P3 stated: \textit{``I wanted to express a longing for freedom, and while modifying the keywords, I gradually thought of a boat which drafting freely (a symbol of freedom).''} 
    She added the keyword ``boat'' to regenerated images, described her thoughts related to the boat, and chose an image of a small boat drifting downstream as an illustration of her post. 
    % ``I wanted to express a longing for freedom, and while modifying the tags, I gradually thought of a boat which drafting freely (a symbol of freedom).''(P3) This was the reason why P3 chose an image of a small boat drifting downstream as an illustration of P3's post.

    \textbf{Expression in image.} We noticed that some users did not modify their text or mentioned that they did not receive inspiration from the image for re-editing their posts. In the interviews, five participants mentioned that the generated images were more suitable for helping them express themselves, so they did not need to modify their text.  ``When expressing my failure in the graduate entrance exam, I got a generated image of a happy person holding an admission letter and another person holding a pen and looking frustrated on an exam paper. I think these two images can well express what I want to say'' (P2). Some users were more concerned about the relevance of the images rather than the text. ``Images can catch one's eyes more quickly than text, so I think the images should represent the content of the post, and I do not need to modify the text'' (P14). This phenomenon aligns with the research in \cite{Rich02}, which states that users tend to use images to express abstract emotions.
    
    % The survey results indicate that nearly all participants who felt that they were better able to express themselves (22 out of 23) expressed satisfaction with their posts. This aligns with the findings of \cite{Peng21, Luo20} and suggests that with the assistance of MentalImager, users achieve a higher level of self-disclosure.

% \begin{table}[h]

% \caption{Analysis of user self-assessment between Baseline and MentalImager, where the p-values ($ *:p < .050, **:p < .010, ***:p < .001$) is reported.}
% \label{tab: 7-2}
% \begin{tabular}{cccc}
% \hline
% Factor                                                                  & Baseline Mean/S.D. & MentalImager Mean/S.D. & P    \\ \hline
% \begin{tabular}[c]{@{}c@{}}The difficulty\\ levle of post\end{tabular}  & 4.58/1.248         & 5.38/1.10              & 0.02 \\ \hline
% \begin{tabular}[c]{@{}c@{}}The degree of\\ self-disclosure\end{tabular} & 4.67/.868          & 5.54/0.72              & ***  \\ \hline
% Emotion relevance                                                       & 4.12/1.72          & 5.20/1.35              & 0.02 \\ \hline
% Topic relevance                                                         & 3.91/1.28          & 5.45/1.21              & ***  \\ \hline
% \end{tabular}
% \end{table}



\subsection{Perceptions towards MentalImager}
As shown in Table \ref{tab: evaluation}, participants were generally positive towards the usefulness of the MentalImager's generated images for facilitating mental health self-disclosure. 
They also deemed its interface easy to use and had a high intention to use it to draft posts to express themselves and seek social support in online mental health communities. 
However, participants also had concerns about the generated images in MentalImager, which are summarized below. 

%     \subsection{System Usability and Features of MentalImager}
%     % In accordance with the defined DRs, we conducted a comparative analysis between the baseline (original community) and the MentalImager system across two dimensions: Self-disclosure levels (DR1) and Image-text relevance (DR2).

%     To establish the reliability of our questionnaire design, we initially employed the Cronbach α coefficient analysis, yielding a coefficient value of α=0.847. This result affirms the questionnaire's reliability in measuring the intended dimensions.
    
%     In reference to the evaluation section mentioned earlier, encompassing three assessment dimensions, we present user ratings across these dimensions in Table \ref{ta}. The outcomes indicate a notably positive user perception of our system. Furthermore, we performed a Wilcoxon signed-rank test, which unveiled significant enhancements in user self-disclosure levels (p=0.03) and the relevance of image-text associations in postings (p=0.01). Interestingly, we also observed a reduction in users' perceived posting difficulty (p=0.24).
    
%     These findings collectively suggest that the MentalImager system has significantly improved users' self-expression capabilities and the relevance of image-text associations in their posts. Additionally, it has concurrently reduced the perceived posting difficulty. For further inquiries or translations, please do not hesitate to contact us.




% \begin{table}[h]
% \caption{Mean and standard deviations of the items measuring the perceived usefulness, easy to use, and intention to use of MentalImager. 7-point Likert Scale, 1 - strongly disagree, 7 - strongly agree.}
% \label{tab: evaluation}
% \begin{tabular}{clcc}
% \hline
% Type                                                                                        & \multicolumn{1}{c}{Factor}                                                                                                                                                              & Mean & S.D. \\ \hline
%                                                                                             & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}The generated images effectively help the poster\\ seek help or express emotions\end{tabular}}                                         & 5.54 & 0.72 \\ \cline{2-4} 
%                                                                                             & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}Using the system effectively helps posters\\ complete posts in mental health communities.\end{tabular}}                                & 5.96 & 1.08 \\ \cline{2-4} 
%                                                                                             & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}The assistant's provided images gave me\\ additional inspiration for writing,\\ making my expression clearer.\end{tabular}}            & 5.33 & 1.09 \\ \cline{2-4} 
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Usefulness for \\ Self-disclosure\end{tabular}} & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}The system quickly accomplishes the task of\\ generating images, saving users' time.\end{tabular}}                                     & 5.33 & 1.58 \\ \hline
%                                                                                             & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}The interaction process is easy\\ even for first-time users.\end{tabular}}                                                             & 5.46 & 1.28 \\ \cline{2-4} 
%                                                                                             & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}The interaction process is easy \\ even for first-time users.\end{tabular}}                                                            & 5.25 & 1.11 \\ \cline{2-4} 
%                                                                                             & {\color[HTML]{374151} It doesn't require a lot of effort to use.}                                                                                                                       & 5.88 & 1.23 \\ \cline{2-4} 
% \multirow{-4}{*}{Easy to use}                                                               & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}The process of obtaining/modifying images\\ is straightforward.\end{tabular}}                                                          & 5.46 & 1.10 \\ \hline
%                                                                                             & {\color[HTML]{374151} \begin{tabular}[c]{@{}l@{}}If I were to post in a mental health community, \\ I would be more inclined to use the assistant \\ to better seek help.\end{tabular}} & 5.54 & 0.72 \\ \cline{2-4} 
% \multirow{-2}{*}{Intention to Use}                                                          & \begin{tabular}[c]{@{}l@{}}Users believe that posts completed with the \\ assistant's help are better understood\end{tabular}                                                           & 5.96 & 1.08 \\ \hline
% \end{tabular}
% \end{table}



    
    % \subsection{Self-disclosure}
    
    % When designing MentalImager, our goal was to encourage users to be more actively involved in the image-generation process and to help them clarify their thoughts to assist in self-disclosure. Regarding this aspect, users provided some positive feedback. Firstly, the majority of users (95\%) felt that they were better able to complete their posts with the assistance of the tool. From the data and interviews, we identified two main areas in which MentalImager was helpful for users.

    % \textbf{Writing Expression:} More than half (58\%) of the users reported that they received inspiration for their writing while either viewing the generated images or during the image generation process. For example, one participant stated, ``I wanted to express the struggles during a period of confusion, but I didn't know how to describe it. When I saw the image of the person standing on top of the mountain, it reminded me of the feeling of striving for one's dreams.''(P10) Consequently, the participant wrote, \textit{``Whenever I feel like giving up, I always think of the original dream.''} Another participant mentioned modifying their wording based on the generated images: ``When expressing the pain caused by the study pressure, I initially used 'stressful'. However, during the process of adjusting the generated image, I received an image of a girl curled up in a corner, which made me think of a 'bottomless pit' (representing endless stress).''(p13) Consequently, the participant changed the title from \textit{Stressful} to \textit{Tremendous pressure of study} and wrote, \textit{``I feel trapped in a bottomless pit of learning.''} We also found that inspiration for modifying tags themselves, which aligns with previous research in 
    % % \qingyu{mental health communities}
    % \cite{Shin22}. For example, P3 chose an image of a small boat drifting downstream as an illustration of P3's post mentioned that \textit{``I wanted to express a longing for freedom, and while modifying the tags, I gradually thought of a boat which drafting freely (a symbol of freedom).''}
    % % ``I wanted to express a longing for freedom, and while modifying the tags, I gradually thought of a boat which drafting freely (a symbol of freedom).''(P3) This was the reason why P3 chose an image of a small boat drifting downstream as an illustration of P3's post.

    % \textbf{Image Expression.} We noticed that some users did not modify their text or mentioned that they didn't receive inspiration for writing. In interviews, users mentioned that they found images more suitable for helping them express themselves, so they didn't need to modify their text: \textit{``When expressing my failure in the graduate entrance exam, I received a happy person holding an admission letter and another person holding a pen and looking frustrated on an exam paper. I think these two images can express what I want to say very well'' (p2)}. Some users were more concerned about the relevance of the images rather than the text: \textit{``Images enter the field of vision more quickly than text, so I think the images should represent the content of the post (so I don't need to modify the text).'' (P14)} We also noticed that this phenomenon aligns with the research in \cite{Rich02}, indicating that users tend to use images to express abstract emotions.
    
    % The survey results indicate that nearly all participants who felt that they were better able to express themselves (22 out of 23) expressed satisfaction with their posts. This aligns with the findings of \cite{Peng21, Luo20} and suggests that with the assistance of MentalImager, users achieve a higher level of self-disclosure.

    % \subsection{Empathy}
    
    % We sought to understand whether users, with the help of MentalImager, wrote more empathetic and engaging posts from two perspectives: the support seeker's viewpoint and the support provider's viewpoint, data was further analyzed using ANOVA method.

    % \textbf{Seeker's Viewpoint}. Firstly, we asked users to self-assess the clarity of their post expression, and notably (as shown in the figure), users rated themselves higher with the assistance of MentalImager. Additionally, we asked users to evaluate the emotional relevance and thematic relevance of the images to their post content. These scores were used for comparative analysis with ratings from the other perspective. From the data, it is evident that with the assistance of MentalImager, users perceived that they were able to express their emotions or needs more clearly and believed they could receive more responses. Particularly, there was an improvement in the visual-textual relevance from the seeker's perspective.
    
    % \textbf{Provider's Viewpoint}. We also invited 6 individuals with experience in posting or commenting on online communities. We grouped the two types of posts generated by the same user in the previous experiment together, and had the raters assess 24 sets of data in 4 dimensions:
    
    % 1. Degree of Empathy: To what extent can you sense the emotions or needs of the poster in this post?
    
    % 2. Image-Text Relevance: Do you think the images in the post are relevant to the theme and emotions in the text?
    
    % 3. Willingness to Reply: Would you be willing to provide support or reply to this post?
    
    % The scoring range for these four dimensions was 1-7, where 1 indicates 'strongly disagree' and 7 indicates 'strongly agree'. In the final results, we found that, according to providers, users' posts written with the help of MentalImager showed a significant increase in empathy, and providers were more willing to respond to these posts. However, there was no significant difference in the evaluation of text-image relevance. This also suggests that seekers and providers have a consistent perception of images, and we consider this as one of the reasons why providers can empathize more with the posts. In interviews, we also found that users always choose images that are more relevant to the emotions or themes of their posts when adding images, otherwise, they would rather not add any images. Considering that MentalImager should provide users with the images that users need (DQ 1) rather than images that match more closely in emotion or topic, it is acceptable that there was no significant improvement in image-text relevance.
    % we found that users preferred posts with images and were more willing to engage with them. Furthermore, the images provided by MentalImager were perceived by providers as having higher emotional and thematic relevance. Additionally, as almost every post with MentalImager's assistance included images, they also received higher empathy scores[with-in, between......] \qingyu{Remember to finish this part}







    % \subsection{Concern}
    % In participant feedback, we found that generative images were less accepted or not significantly helpful for some users in certain aspects. In this section, we provide some design concerns based on the results.

    \textbf{Style of the generated image.} Our model only supports generating images in an animated style to avoid infringing on personal or organizational rights. However, for seven users, this image style is not of their interest. For example, P1 said, \textit{``I prefer images related to movies or songs; the animated style is too monotonous for me.''} 
    % System designers could consider allowing users to choose from a wider range of styles. 
    Furthermore, five users mentioned that generative images might not work well for extreme topics: \textit{``When I was writing a post about depression, the system provided me with some dark-themed images that made me feel frightened''} (P20). 
    This could be due to the negative keywords as the input to the text-to-image generative model and raise the need to the control of generated content for supporting people with mental health concerns.
    % We consider that in extreme topics, the keywords extracted by the model are also negative, leading to negative feedback from users. Designers might consider filtering out some extreme topics or vocabulary to protect users from the model's negative impact.

    \textbf{Quality of the generated images.} Users mentioned that the model sometimes returns irrelevant images or generates low-quality images for certain topics, which negatively affects their impression of the system. 
    \textit{``When I was discussing some traditional issues in China, I did not receive images that perfectly matched my ideas'' (P6).} Therefore, we suggest system designers provide the text-to-image model with more vocabulary information to reduce this issue.
    This issue could be due to the limited training data that contain the keywords about mental health self-disclosure and yield the need to fine-tune the text-to-image generative models. %, affecting the quality of images generated.
    
    \textbf{Keyword Extraction.} Since we used the TF-IDF algorithm to extract keywords in our experiment, it has limitations compared to large language models or deep learning techniques for keyword extraction. 
    It can not guarantee that every extracted keyword is closely related to the user's text, especially when the user's initial expression is poor. 
    \textit{``When drafting the post, I vent my emotions in a casual and scattered way, and the extracted keywords were not correctly matched with my thoughts''} (P21). 
    The post with multiple topics (\eg study, sleep, flight, and girlfriend) also makes it difficult to extract keywords that are closely related to a topic, which could reduce the performance of the text-to-image generation model. 
    % , especially if these keywords are unfamiliar to the text-to-image model, which can further amplify errors. Therefore, we suggest that designers consider improving the keyword extraction method to accommodate users with various writing skill levels.
        




==> sections/figures.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{figures/post.png} 
  \caption{One of the posts used for user rating. The left side shows the post's title and content, while the right side displays the images obtained from the four methods: (a) image from Google images search, (b) content-based method, (c) without extra keywords method, and (d) with extra keywords method. The keywords of (c) are: \textit{broken,  happy, depressed, pity, displaying self pity, 0 self confidence, someone please get, said,works, understands}. For (d), in addition to all the keywords from (c), there are additional emotion keywords obtained through BERT analysis: \textit{sadness}, as well as topic keywords extracted from the title: \textit{hopeless}.
}
  \label{fig:post}
\end{figure}


==> sections/pzh_new_outline.tex <==
\peng{

% \section{Study II: Impacts of Generated Images on Mental Health Self-Disclosure (RQ2)}
% Transition sentence here
% \subsection{Participants}

% \subsection{Task and Procedure}

% \subsection{Measures}

% \subsection{Ethical Concerns}

% \subsection{Analyses and Results}

% \subsubsection{Self-disclosure outcome}

% \subsubsection{Self-disclosure experience}

% \subsubsection{Perceptions towards MentalImager}

\section{Discussion}
\begin{itemize}
    \item Talk about how our findings link to previous work and contribute to the CSCW community. 
\end{itemize}
\subsection{Design Considerations}
Try to raise three design considerations derived from our study results.

\subsection{Limitations and Future Work}
}


